Constraining Extended Scalar Sectors at the LHC and beyond

We give a brief overview of beyond the Standard Model (BSM) theories with an extended scalar sector and their phenomenological status in the light of recent experimental results. We discuss the relevant theoretical and experimental constraints, and show their impact on the allowed parameter space of two specific models: the real scalar singlet extension of the Standard Model (SM) and the Inert Doublet Model. We emphasize the importance of the LHC measurements, both the direct searches for additional scalar bosons, as well as the precise measurements of properties of the Higgs boson of mass 125 GeV. We show the complementarity of these measurements to electroweak and dark matter observables.

==> higho.tex <==
\section{A brief note on higher-order corrections and gauge-parameter independence}
\htr{(TS: I think we should remove this section.)}
\htb{[TR i entered this, but mb we have to cut it out. i think i already reached the page limit, and we still wait for tims plot. and i have to add many acknowledgements re funding... we will see. ;-)]}
In recent years, a lot of effort has gone into the calculation of higher-order electroweak corrections for models with extended scalars sectors, with a special emphasis on the investigation of gauge-parameter independence of predictions for physical quantities (see \cite{Nielsen:1975fs,Fleischer:1980ub,Gambino:1998ec,Kniehl:2000rb,Yamada:2001px,Espinosa:2002cd,Actis:2006ra} for similar early discussions). For brevity, we only list the relevant publications and point the reader to these for further details\footnote{We omit the discussion of models with extensions exceeding the scalar sector, as e.g. supersymmetric models.}
\begin{itemize}
\item{}Gauge-parameter independence of physical observables for the renormalization in the electroweak sector within the singlet extension has first been discussed in \cite{Bojarski:2015kra}; subsequent studies for this and other BSM scenarios were presented in \cite{Krause:2016oke,Denner:2016etu,Krause:2016xku,Kanemura:2017wtm,Altenkamp:2017ldc,Denner:2017vms,Krause:2017mal,Altenkamp:2018bcs}.
\item{}Several of these studies are now available within generic tools that can be used by the LHC collaborations, cf. \cite{Denner:2017vms,Denner:2017wsf,Altenkamp:2018bcs,Djouadi:2018xqq}
\end{itemize}
Therefore, higher-order electroweak corrections in the singlet extension and other models mentioned above are now understood from a theoretical viewpoint and can readily be included in the respective LHC analyses.

